L-Violating Supersymmetry - Implementation in PYTHIA and study of LHC discovery potential

In the Minimal Supersymmetric Standard Model (MSSM), the simultaneous appearance of lepton and baryon number violation causes the proton to decay much faster than the experimental bound allows. Customarily, a discrete symmetry known as R-parity is imposed to forbid these dangerous interactions. This work begins by arguing that there is no deep theoretical motivation for preferring R-parity over other discrete symmetries and continues by adopting the MSSM with baryon number conservation replacing R-parity conservation. For the purpose of studying the influence of the consequent lepton number violating interactions, 1278 new decay channels of supersymmetric particles into Standard Model particles have been included in the PYTHIA event generator. The augmented event generator is then used in combination with the atlfast detector simulation to study the impact of lepton number violation on event topologies in the ATLAS detector, and trigger menus designed for LV-SUSY are proposed based on very general conclusions. The subsequent analysis uses a combination of primitive cuts and neural networks to optimize the discriminating power between signal and background events. In all scenarios studied, it is found that a $5\sigma$ discovery is possible for cross sections down to $10^{-10}$ mb with an integrated luminosity of 30 fb$^{-1}$.

==> APPENDICES/neural.tex <==
\section{Neural Network Learning Rules\label{app:neural}}
The neural networks employed in this work all learn by adjusting their
synaptic weights, temperatures, and biases at the end of each pass over the
learning samples in the direction which minimizes the error. This aprroach is
known as the \emph{gradient descent} method \cite{mcclelland89}. As the name
implies, the learning rule is defined by taking a step in weight space in the
direction of the gradient of the (squared) error:
\begin{equation}
p \to p + \Delta p = - \alpha\frac{\partial e^2}{\partial p} = p + 2\alpha e
\frac{\partial \mathcal{O}}{\partial p}
\end{equation} 
where $p$ represents any of the variable parameters in the network, 
$e=t-\mathcal{O}$ is the error on the output (target output: $t$, obtained
output: $\mathcal{O}$), and $\alpha$ is a learning
rate parameter. This rule does not necessarily have to be applied after every
event in the learning sample. In order to wash out sharp, irregular 
changes called for from
extreme events in the distributions, 
we do better in accumulating the parameter changes over some processing
period without invoking them. After the period, the \emph{accumulated} change to each
parameter is invoked, and the accumulated error is reset. 
In order to get as little statistical noise in
the parameter changes as possible, the period is set to be the number of
events in the learning sample. Denoting event number by $n$,
the learning rule above becomes:
\begin{equation}
p \to p + \Delta p = p + 2\alpha \sum_ne(n)
\frac{\partial \mathcal{O}(n)}{\partial p}
\end{equation} 
One further improvement can be made on the learning rule. Seeing as two
successive changes to the parameters of the network 
often go in roughly the same direction in parameter
space, something which often increases the learning speed of the network:
\begin{equation}
p \to p + \Delta p = p + 2\alpha \sum_ne(n)
\frac{\partial \mathcal{O}(n)}{\partial p} + \beta \Delta p^{\mathrm{last}}
\label{eq:learnrule}
\end{equation} 
where $\Delta p^{\mathrm{last}}$ is the change which was made the previous
period, and $\beta<1$ specifies the ``inertia'' of the system. 
We are now ready to specify the learning rules for each of the parameters of
the network in fig.~\ref{fig:netlayout}. 
These can be easily derived. 
\begin{eqnarray}
\frac{\partial \mathcal{O}}{\partial o_j} 
& = & \frac{H_j}{N_{\mathrm{hid}}} \\
\frac{\partial \mathcal{O}}{\partial w_{ij}} & = & \frac{o_j}{N_{\mathrm{hid}}} 
H_j(1-H_j)I_i \\
\frac{\partial \mathcal{O}}{\partial \epsilon_j} & = & o_jH_j(H_j-1)\\
\frac{\partial \mathcal{O}}{\partial \delta_i} & = &
\frac{I_i(1-I_i)}{T_i}\sum_j o_jH_j(H_j-1)w_{ij} \\
\frac{\partial \mathcal{O}}{\partial T_i} & = &
\frac{\mathrm{In}_i}{T_i^2}I_i(1-I_i)\sum_jo_jH_j(H_j-1)w_{ij}
\end{eqnarray}
Replacing these quantities back into eq.~(\ref{eq:learnrule}) directly 
yields the required learning rules.


==> INTRO/preface.tex <==
\pagestyle{headings}
\addcontentsline{toc}{section}{Preface \& Outline}
\noindent\textbf{\Large Preface}\vspace*{5mm}\\
Thales, native to the Ionian city of Miletus and first of the famous Milesian
Trio is traditionally credited with beginning the greek tradition for natural
philosophy in the sixth century BC \cite{luce92}. The essence of the way of
thought begun by Thales and his two contemporaries in Miletus, Anaximander
and Anaximenes, has become the very cornerstone of all the science of physics
(from the greek \emph{phusis}: Nature or that which has not been made by
man). This thought can be expressed as a belief that the world is not
governed by the wills and vanities of Gods but instead by immutable laws
arising from fundamental relationships between some basic elements of
Nature. In Greece, the nature of these laws and elements was predominantly
arrived at through speculation, a technique still in frequent use, though
most often combined with the Gallilean view which gives the experiment
ultimate judgement.  I shall not here recapitulate to any extent the science
of physics, yet for the inexperienced reader, I will briefly set the stage on
which the present work has been performed.

The Democritian hypothesis that Nature, at the most fundamental level,
consists of a set of indivisible basic elements is still all-dominant in
physics. Today, the twilight of possible discoveries is found deep within the
atomic nucleus and even deeper, within the nucleons themselves, at the
smallest length scales yet probed by any experiment. In the continued quest
for Democritus' elements, we have reached objects which, if size they have,
are about a billionth of a billionth of a decimeter across, a billionth the
size of a normal atom. We do not yet know whether these objects have any
internal structure. They are the quarks and leptons (6 of each) which
constitute all matter known to us and the bosons which carry the four
fundamental forces of Nature known to us.  The fourth force, gravity, is,
however, still lacking a complete description.

Combined, these particles and the interactions between them are incorporated
in a theoretical framework known as the Standard Model of particle physics
(the SM). We know, however, that this model cannot be the whole story, and
therefore a number of speculations on the possible existence of more hitherto
undiscovered properties of Nature has arisen. That Nature could contain a
special symmetry known as supersymmetry is one of these speculations, and our
belief in it is spurred on by its providing an elegant solution to a
fundamental problem in the Standard Model connected with the nature of mass
and by its being a key ingredient in many of the attempts to provide a
quantum description of gravity. A natural question to ask is then why we
haven't seen the effects of this symmetry yet. How can a symmetry that we
postulate as fundamental to Nature remain hidden from us so thoroughly? The
answer to this is that the symmetry could be broken in such a way that the
symmetry itself would only be directly manifest at length scales about ten
times smaller (which is the same as energy scales ten times lerger) than the
ones we have reached so far. The exact nature of supersymmetry and its
consequences are described below, yet there is one more issue of relevance to
this work that must first be introduced.

\paragraph{The Monte Carlo method:} In present-day high energy experiments, an
enormous amount of physical processes occur from the initial
state in time when two quantum particles (perhaps
also possessing internal structure) approach each other at ultra-relativistic
speeds inside the
beam pipe of some high-energy accelerator to the point, after the
interaction, when particle tracks, energy depositions, detector
status etc.\ are read our from the detector. Furthermore, the
probabilistic nature of quantum mechanics ensures that any given
initial state can result in a truly enormous number of possible
final states. It is therefore a central task for the
experimentalist to reconstruct what \emph{actually} happened in
each event recorded, and to design a detector that enables a
distinction between "interesting" and "uninteresting" events. The
theorist faces similar problems. To enable a comparison with
experiment, the theory must deliver predictions of experimental
observables. It is therefore not enough simply to study and
calculate the elementary interactions contained in a given
theory; these are only very rarely directly visible to the
experiment. In most cases, a full, analytical calculation of
everything that goes on between some initial state and some final
state is simply out of the question. It is here that Monte Carlo
generators come into the picture. The power of computers to
perform repetitive tasks according to specific rules combined
with the statistical Monte Carlo method has become an
indispensable tool in comparing theory with experiment.

In Monte Carlo implementations, the elementary processes that
occur and about which we wish to extract information are dressed
with all the `junk' that occurs before, during, and after the
interaction, thus simulating a real interaction between physical
particles. Add to this a simulation of how the detector apparatus
works (\emph{no} detector catches everything), the generated
event has all the likeliness of a real event, except for the fact that in
\emph{this} case we have full knowledge of what the fundamental
process was, and so the efficiency of particle identification algorithms
etc.\ which are used in the real experiment can be tested, enabling an
evaluation of our capability to interpret the observed data in
terms of the underlying theory. The limitation is, of course,
that it is impossible to include \emph{all} possible effects that
can occur in a physical interaction, and so one should never
blindly trust MC results without a critical analysis of whether
all important effects have been taken into account. Exercising
caution on this point, MC simulations can be extremely useful in
interpreting observed phenomena, in optimizing detector design and
in finetuning the analysis strategies used in the actual experiment.

\paragraph{Outline:}
%\addcontentsline{toc}{section}{Outline}
In the introduction, a brief account of the theoretical
considerations fuelling 
the widespread belief in supersymmetry is given, together with an
introduction to that particular class of supersymmetric theories
called $R$-parity violating which comprises the subject of this
thesis. In section \ref{sec:model} the details of the supersymmetric model
adopted in this work are explained. The $L$-violating decays of
supersymmetric particles 
and their implementation in \pythia\ are discussed in section
\ref{sec:lspdecays}. 
\SIP
\cleardoublepage


==> LVDECAY/pythia.tex <==
\subsection{Implementing L-violating decays in PYTHIA}
\label{sec:pythia}
The original work performed in this thesis has noot been to present an
introduction to supersymmetry or to review the motiviations (or lack of same)
for the discrete symmetries thought to protect the proton. Nor has it
been to calculate Feynman diagrams to obtain the decay matrix elements. When
these calculations and arguments for and against have now been presented, it
has been with one specific goal in mind -- that the reader should by now be
convinced 
of what I believe is the necessity of studying \LV-SUSY scenarios,
and that the reader should have been
confronted with enough phenomenological as well as computational basis that
he could take part in this study himself. The original work, then, that has
so far been contained within these pages is the 
F77 source code for the subroutines which
have been added to \pythia\ in the course of this work. Since this material
is intended for general use, a few comments are necessary regarding the
parameters that an eventual user would have to be familiar with.
\paragraph{Switches \& Parameters that should be set by the user in the
\pythia\ calling program}
\begin{itemize}
\item IMSS(13): $\lambda$ couplings. Default is off (=0).
\begin{itemize}
\item (=0): $\lambda$ couplings off. 
\item (=1): All allowed couplings set to fixed value given by
RMSS(31). Default value for RMSS(31) is 0. 
\item (=2): Couplings set to ``natural values'',
$\lambda_{ijk}\propto\sqrt{m_im_jm_k/(126\GeV)^3}$, as defined in
\cite[eq.~(17)]{hinchliffe93}, 
giving a hierarchical structure in generations. RMSS(31)
is here used to give the constant of proportionality. If the user does not
have other specific wishes, its value should be set to 1 when using 
this scenario.
\item (=3): The program initializes with default values ($\lambda_{ijk}=0$),
but expects the user to enter all non-zero couplings by hand into the
RVLAM(I,J,K) array in the calling program. 
\end{itemize}
\item IMSS(14): $\lambda'$ couplings. Default is off (=0).
\begin{itemize}
 \item (=0): $\lambda'$ couplings off. 
 \item (=1): All couplings set to fixed value given by RMSS(32). Default
 value for RMSS(32) is 0. 
 \item (=2): Couplings set to ``natural values'',
$\lambda'_{ijk}\propto\sqrt{m_im_jm_k/(126\GeV)^3}$, as defined in
\cite{hinchliffe93}, with the constant of proportionality given by
 RMSS(32). If the user does not
have other specific wishes, its value should be set to 1 when using 
this scenario.
\item (=3): The program initializes with default values ($\lambda'_{ijk}=0$),
but expects the user to enter all non-zero couplings by hand into the
RVLAMP(I,J,K) array in the calling program. 
\end{itemize}
\item (IMSS(15)): Should be reserved for $\lambda''$ couplings on/off
together with RMSS(33).  
\item IMSS(16): Precision for the phase space integrations. $10
\times$IMSS(16) = \# integration steps. Default is IMSS(16)=5.
\item PYMSRV : This is the commonblock in \pythia\ where the $L$-violating
couplings reside; the $\lambda_{ijk}$ couplings are stored in RVLAM(i,j,k),
and the $\lambda'_{ijk}$ in RVLAMP(i,j,k). Space has been reserved for an
eventual future study of $B$-violation in the RVLAMPP(i,j,k) array which is
intended to store the $\lambda''_{ijk}$ couplings.
\end{itemize}
\paragraph{Subroutines and functions handling $R$-violation inside \pythia}
\begin{itemize}
\item PYRVST : Subroutine to print information about semi-inclusive branching
ratios and coupling values. Called from PYSTAT if R-Violation has been turned 
on (IMSS(13)=1 or IMSS(14)=1).
\item PYRVSF : Subroutine to calculate \RV\ decay widths of sfermions based
on the selected SUSY scenario and coupling values. If there is no phase space
available for a given mode, the width for that mode is set to zero and
\pythia\ is told to ignore the mode completely. 
\item PYRVN  : Same as above for \RV\ decays of neutralinos.
\item PYRVCH : Same as above for \RV\ decays of charginos.
\item PYRVF1, PYRVF2, PYRVF3, PYRVIN, PYRVR, PYRVS, PYRVRS, PYRVYZ, PYRVSM,
and PYRVSB : Auxiliary routines and functions to assist in the calculation of
often repeated quantities in the three main routines. A small description of
each is provided in the source code.
\end{itemize}
In addition, a consistency check has been added to the routine which
diagonalizes the neutralino mass matrix (PYEIG4) so that error messages will
be printed if the off-diagonal elements of the diagonalized matrix
(recomputed from the original matrix and the diagonalizing matrix given by
the routine) are larger than $10^{-6}$ or if the diagonal elements calculated
by brute force deviate by more than $10^{-6}$ from the values in the mass
vector given by the routine. This does not encumber the performance of
\pythia\ in any way, since the matrix needs to be diagonalized only once for
each run. 

\paragraph{Warnings and error messages:}
Since the numerical integrations over phase space are only approximately
correct and the approximations can break down, e.g.\ due to $t$ quark 
threshold effects, a number of devices for testing the reliability of the
methods used have been implemented in the code. This should give some
security towards not getting completely wrong results without accompanying
warnings. 
\begin{itemize}
\item \texttt{PYRVN \mbox{(or \texttt{PYRVCH})} warning: Interference terms
in $\ti{a}\to b\ c\ d$\ AVG = < NN.N\% >}. Since the integration over
interference terms is rather crude, rapidly varying interference
contributions are dangerous if the contributions are not small. To test
whether the contributions are small (on average), a
counter has been placed inside the integration which, after each integration
step, is increased by the total contribution from interference terms at that
step divided by the total contribution of non-interference terms at that
step. After the integration, when divided by the number of integration steps,
this counter will have the value 1 if the interference terms are, on average,
equal to the non-interferent terms. It will be less than 1 if the
interference terms are smaller. This message will
be printed if the interference terms give a contribution which is, on
average, larger than 25\% of the non-interferent contributions. One should
then check carefully whether the interference terms could be rapidly
varying in which case there is no other option but to dramatically increase
the number of integration steps (using IMSS(16)).
\item \texttt{PYRVN \mbox{(or \texttt{PYRVCH})} : Very large interference
terms encountered in $\ti{a}\to b\ c\ d$. \textsf{X} times resonant
terms}. If, for any point in the numerical integration, 
the sum over interferences reaches more than ten times 
the sum over resonance contributions, this warning 
message is immediately printed. For the reasons given above, this should be
considered very serious, and the number of integration steps should be
increased dramatically (using IMSS(16)).
\item \texttt{PYRVN \mbox{(or \texttt{PYRVCH})} : X($i$) Limit consistency
check failed in $\ti{a}\to b\ c\ d$}. After the numerical integration, it is
checked whether the stepping of $dx$ has resulted in a correct $x_{max}$. If
not, this error is printed. Also performed for $Y$ integrations. 
\item \texttt{PYRVN \mbox{(or \texttt{PYRVCH})} : Negative Width in
$\ti{a}\to b\ c\ d$}. 
If the width calculation
results in a negative number, this error is printed. It is most often the
result of large negative interference contributions and can be cured by
increasing the precision.
\end{itemize}
It should be noted that most of the problems with interference contributions
only appear in the low-mass 
region of parameter space where the $t$ quark threshold can lead to large
interference contributions for the low-mass gauginos. Since these modes are
kinematically suppressed (due to the large $t$ mass) one can, in most cases,
completely disregard these problems. The widths may be wrong, but as long as
one checks explicitly that they are still small compared to processes not
involving the $t$ quark, the effect is negligible.

\subsubsection{Resonant decay treatment}
\label{sec:resdec}
Each time a physical particle is
generated in \pythia, a random mass is calculated, distributed according to
the Lorentz profile for that particle. As decay widths and therefore branching
fractions depend on the mass of the incoming particle\footnote{This becomes
especially important when some of the channels contain particles with masses
close to 
the decaying particle's mass. In that case, there will be a threshold where
only particles above the threshold mass can decay via that channel.}, 
the most detailed
method for determining in which channel the particle will decay is to
calculate its
widths to all available channels at that mass and from them determine the
branching fractions. This is feasible
for low-mass particles with few and/or simple decay channels, and so every
time a $W$ boson, for example, decays in \pythia, its branching fractions are
evaluated at the specific mass of that $W$. For supersymmetric particles
with hundreds of decay channels and many adjustable SUSY parameters entering
the calculations, this 
method would be very time consuming with \emph{all} decay widths having to be
recalculated each time a particle is generated. Instead,
an approximate method is used. All branching fractions are evaluated once and
for all at the resonance mass during each program execution. This saves CPU
time, yet
it has the potential danger that some of the sparticles produced in the
generator have masses that could be lower than some threshold where some
channel reaches zero phase space. Allowing such a sparticle to decay into
that channel would result in violation of energy conservation. \SIP

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 

